Analyzing Commonsense Emergence in Few-shot Knowledge Models

Recently, commonsense knowledge models - pretrained language models (LM) fine-tuned on knowledge graph (KG) tuples - showed that considerable amounts of commonsense knowledge can be encoded in the parameters of large language models. However, as parallel studies show that LMs are poor hypothesizers of declarative commonsense relationships on their own, it remains unclear whether this knowledge is learned during pretraining or from fine-tuning on KG examples. To investigate this question, we train commonsense knowledge models in few-shot settings to study the emergence of their commonsense representation abilities. Our results show that commonsense knowledge models can rapidly adapt from limited examples, indicating that KG fine-tuning serves to learn an interface to encoded knowledge learned during pretraining. Importantly, our analysis of absolute, angular, and distributional parameter changes during few-shot fine-tuning provides novel insights into how this interface is learned.

==> figures/decoding.tex <==
\begin{comment}
\begin{table*}%[!htbp]
\begin{center}
\begin{tabular}{lc|ccc}
\textbf{Methodology} & \multicolumn{1}{l}{\makecell{\textbf{2-Gram} \\ \textbf{Unique \%}}} & \multicolumn{1}{l}{\textbf{BLEU-2}} & \multicolumn{1}{l}{\textbf{Accept \%}} \\ \toprule
Greedy decoding & 23.5 & 28.6 & 84.6 \\ 
Beam search, $b = 10$ & 22.9 & 28.9 & 85.2 \\
Stochastic beam search \cite{Kool2019StochasticBA}, $b = 10$  & 27.0 & 27.9 & 85.9 \\ \midrule
Sampling, $t = 0.3$ & 30.1 & 28.2 & 83.6 \\
Sampling, $t = 0.7$ & 30.7 & 27.8 & 85.0 \\
Top-k, $k = 50$ & 33.1 & 24.3 & 83.5 \\
Top-p \cite{Holtzman2020TheCC}, $p = 0.3$ & 31.2 & 28.9 & 85.8 \\
Top-p \cite{Holtzman2020TheCC}, $p = 0.7$ & 32.7 & 29.3 & 85.8 \\ \bottomrule
\end{tabular}
\end{center}
\caption{Decoding method effect on variability and verifiability trained on full training set.}
\label{table:decoding}
\end{table*}
\end{comment}

==> figures/decoding_few.tex <==
\begin{comment}
\begin{table*}%[!htbp]
\begin{center}
\begin{tabular}{lc|ccc}
\textbf{Methodology} & \multicolumn{1}{l}{\makecell{\textbf{2-Gram} \\ \textbf{Unique \%}}} & \multicolumn{1}{l}{\textbf{BLEU-2}} & \multicolumn{1}{l}{\textbf{Accept \%}} \\ \toprule
Greedy decoding & 32.4 & 19.3 & 82.1 \\ 
Beam search, $b = 10$ & 30.9 & 18.6 & 82.3 \\
Stochastic beam search \cite{Kool2019StochasticBA}, $b = 10$  & 33.0 & 18.4 & 85.3 \\ \midrule
Sampling, $t = 0.3$ & 33.2 & 18.9 & 84.0 \\
Sampling, $t = 0.7$ & 33.5 & 18.5 & 84.1 \\
Top-k, $k = 50$ & 35.4 & 17.3 & 83.0 \\
Top-p \cite{Holtzman2020TheCC}, $p = 0.3$ & 34.8 & 19.4 & 85.1 \\
Top-p \cite{Holtzman2020TheCC}, $p = 0.7$ & 35.0 & 19.6 & 85.1 \\ \bottomrule
\end{tabular}
\end{center}
\caption{Decoding method effect on variability and verifiability trained on 30 examples per head.}
\label{table:decoding}
\end{table*}
\end{comment}

==> figures/generations_fewvsfull.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[t]
\resizebox{\linewidth}{!}{
\begin{tabular}{llll}
\textbf{Head} & \textbf{Relation} & \textbf{Generated Tail (Few-Shot)} & \textbf{Generated Tail (Full)} \\ \toprule
nail & AtLocation & construction site & floor \\ \midrule
state highway & ObjectUse & statewide transportation & drive across state \\
video camera & ObjectUse & video recording & make a movie \\ \midrule
PersonX takes it to the vet & HinderedBy & \makecell[l]{PersonX doesn't have\\money to pay the vet} & the vet closed up shop. \\
PersonX makes PersonY very sick & HinderedBy & \makecell[l]{PersonX isn't\\close to PersonY.} & \makecell[l]{PersonX is\\not contagious.} \\ \midrule
PersonX finds another job & isAfter & PersonX leaves job & PersonX gets fired \\ \midrule
PersonX falls ill & isBefore & PersonX feels sick & PersonX takes medicine \\ \midrule
\makecell[l]{PersonX gets a call\\for an interview} & xAttr & qualified & hopeful \\
\makecell[l]{PersonX wants to\\learn how to swim} & xAttr & \makecell[l]{PersonX isn't confident\\in the water} & persistant \\ \midrule
PersonX falls ill & xEffect & is hospitalized & \makecell[l]{PersonX spends\\time recovering} \\
PersonX sprays by a skunk & xEffect & PersonX will be sick & \makecell[l]{has to bathe\\in tomato soup} \\ \midrule
PersonX gets milk & xIntent & to drink milk & to drink something \\
PersonX works really hard & xIntent & to be appreciated & to be successful \\ \midrule
PersonX misses class & xNeed & to have a valid excuse & to not go to school \\
PersonX pumps PersonX's gas & xNeed & to have a gas pump & get out of car \\ \midrule
PersonX notices a strange smell & xWant & to investigate the smell & to find the smell \\
PersonX throws a frisbee & xWant & to catch the frisbee & to run after it \\
PersonX wants to learn how to sing & xWant & to take voice lessons & to join a choir \\ \bottomrule
\end{tabular}
}
\caption{Generations produced by Few-Shot COMET (T5) (trained on 3 examples) and Fully Supervised COMET (T5), trained on the entirety of ATOMIC-2020 (about 1 million examples). Despite only seeing a few examples, Few-Shot COMET (T5) is able to produce a variety of generations across relation types.}
\label{table:generations}
\end{table*}

==> figures/illustration_induction.tex <==
\begin{figure}[t]
\centering
  \includegraphics[width=0.5\textwidth]{images/example_induction.pdf}
  \caption{We investigate two training schedules: 1) Pretraining on the seed relations, followed by training on $n$ examples of the target relations (\legendplus); 2) Training only on $n$ examples of the target relations (\legenddot).}
  \label{fig:example_induction}
\end{figure}

==> figures/illustration_tails.tex <==
\begin{figure}[h]
\centering
  \includegraphics[width=0.5\textwidth]{images/example_tails.pdf}
  \caption{Illustration of sampling $n = 3$ tuples from a knowledge graph for the same relation by prioritizing diverse head entities (\legendplus) or multiple tail entities per head entity (\legenddot).}
  \label{fig:example_tails}
\end{figure}

==> figures/illustration_templates.tex <==
\begin{figure}[t]
\centering
  \includegraphics[width=0.5\textwidth]{images/example_templates.pdf}
  \caption{Illustration of knowledge model prompting. The commonsense KG relation is mapped to a natural language template that more closely resembles an input the model has learned to process from pretraining.}
  \label{fig:example_templates}
\end{figure}

==> figures/induction.tex <==
\begin{figure}[t]
\centering
  \includegraphics[width=0.5\textwidth]{images/induction.pdf}
  \caption{Comparison of few-shot training only on target relations (\legendplus) compared to pretraining on seed relations in the \atomicTT{} training set, and then few-shot training on the target relations (\legenddot). We also show the effect of limited pretraining on non-target relations ($n$ per relation; \legendtriangle).}
  \label{fig:induction}
\end{figure}

==> figures/tails.tex <==
\begin{figure}[t]
\centering
  \includegraphics[width=0.5\textwidth]{images/tails.pdf}
  \caption{Comparison of training on examples with diverse head entities (\legendplus) or multiple tail entities per head (\legenddot). Our results suggest that example breadth is more important for training knowledge models than example depth.}% -- which is especially prevalent in fewer-shot settings.}
  \label{fig:tails}
\end{figure}

% \begin{figure}[t]
% \centering
%   \includegraphics[width=0.5\textwidth]{images/example_tails.png}
%   \caption{Illustration of an $N = 3$ knowledge graph in both the single tail (blue) and diverse tail (red) settings.}
%   \label{fig:example_tails}
% \end{figure}

==> figures/weightdiffs.tex <==
\begin{comment}}
\begin{figure*}[t]
\centering
  \includegraphics[width=\textwidth]{images/weightdiffs.png}
  \caption{Weight differences.}
  \label{fig:induction}
\end{figure*}
\end{comment}

==> sections/5x-decoding-studies.tex <==
\begin{comment}

\section{How should we make knowledge models talk?}

\input{figures/decoding}
\input{figures/decoding_few}

Separate to \textit{quality} generations, a knowledge model should be also able to produce \textit{diverse} generations - humans, for example, are able to produce several tails per head. This is critical for knowledge graph coverage, since a large amount of tails can be attributed to a single head. However, a formal exploration in diverse commonsense generation is missing in previous work. Therefore, we produce the first such experiments here.

We consider various generation strategies, namely top-k, top-p, greedy, beam search, temperature sampling, and stochastic beam search. We fix the generation length to 128 tokens, but allow the model to generate a stop token before then. We perform three generations per head with different seeds for all strategies that make stochastic decisions, and report average values.

Table \ref{table:decoding} shows our results. Since it is especially important to assess generation quality here, we run human evaluation for all tuples here. In addition to accuracy metrics, we also consider the following metrics to capture the repetitiveness of the generation:

\begin{itemize}[wide, labelwidth=!,listparindent=0pt, labelindent=0pt,noitemsep,topsep=1pt,parsep=2pt,leftmargin =*]
\item \textit{Distinct 1-gram and 2-grams} is the average number of distinct 1-grams and 2-grams present in the generated text. We include 1-grams to capture diversity in tails with less than two words per tail, which is common for some relations \cite{Vijayakumar2016DiverseBS}.

\item \textit{2-gram proportion} is the average ratio of distinct 2-grams in machine and human generated text \cite{Holtzman2020TheCC}.

\end{itemize}

As expected, beam search produces generations that are less diverse than greedy but are higher quality. Top-p produces the most diverse generations, followed by top-k. Surprisingly, there is not a trade-off between diverse generations and generation quality. Top-p decoding, for example, produces both generations that are judged by high quality by human annotators and most diverse.
\end{comment}

==> sections/5x-example-studies.tex <==
\section{How should we annotate new knowledge relations?}
% \label{sec:data_studies}

% \input{figures/illustration_tails}
% \input{figures/tails}

\input{figures/illustration_induction}
\input{figures/induction}

\input{figures/weightdiffs}

% In this section, we design two studies to explore the effect of training set construction on few-shot learning of commonsense knowledge models, guiding future annotation efforts in commonsense knowledge graphs. First, we compare the tradeoff of example breadth and example depth by evaluating the learning improvement from training on different head entities for the same relation (\ie, breadth) or different tail entities for the same head entity (\ie, depth). Second, we explore whether pretraining on other relations in the graph can help few-shot transfer for a specific target relation, simulating a situation where we may want to learn a new commonsense relation in an online manner.

% \subsection{Heads or Tails: Example Breadth vs. Example Depth}

% \label{ssec:headsortails}

% % \subsubsection{Finding}

% \textbf{Training knowledge models with diverse heads, rather than many tails per head leads to better few-shot learning performance (Figure \ref{fig:tails}).
% }

% % \paragraph{Method}

% \noindent In this setting, we compare two strategies for sampling examples for few-shot learning (Figure \ref{fig:example_tails}). In the first, we sample diverse head entities (\ie, unique seed instances), and limit any head entity to be sampled only once in the few-shot training set. In the second strategy, we sample multiple tail entities per head entity. Here, the model can learn from a richer set of commonsense relationships for each head entity, but at the expense of learning from fewer head entities overall. We sample head entities that are linked to at least 5 tail entities through the same relation in \atomicTT{}, and collect all tails for those sampled heads.

% \paragraph{Findings}

% In Figure \ref{fig:tails}, we see a large empirical gain when training on diverse heads rather than training on more tails per head.\footnote{We do not endorse extrapolating these findings to other common formulations of the ``heads or tails?'' question.} While this difference is most notable for small $n$ (\ie, more extreme few-shot settings), a gap persists across all values of $n$. Consequently, when annotating commonsense knowledge graphs for few-shot transfer, we advise annotating diverse head entities for each relation, rather than annotating multiple inferences for the same head entities (\eg, training with contrast sets; \citealp{gardner-etal-2020-evaluating}). 

\subsection{Does knowledge of other relations help to learn a \textit{new} relation?}

\label{ssec:kpretrain}

% \subsubsection{Finding}

\textbf{Models benefit from pretraining on the other relations in \atomicTT{} in ultra few-shot settings. As the number of examples for a relation increases, pretraining no longer helps (Figure \ref{fig:induction}).
}

% \paragraph{Method}

\noindent In this study, we select a subset of 6 relations from \atomicTT{} as the few-shot set. % (2 relations related tfrom physical, 2 from event-centered, and 2 from social categories in ATOMIC2020). 
Then, we pretrain the knowledge model on all examples of the remaining relations in \atomicTT{}. As before, we use natural language prompts to represent relations, as we want knowledge about relations to transfer between them, which symbolic relation representations would hinder. We then perform few-shot training on the set-aside relations using $n$ examples from each relation. Here, we cap our study at a maximum $n = 300$, as we see no improvement from pretraining with larger $n$. We compare these results to a baseline trained on $n$ examples from the set-aside relations with no pretraining. Additionally, we compare with a model trained on $n$ examples of both the set-aside relations and the seed relations in \atomicTT{}.

\paragraph{Findings}

We find that when more than 30 examples of a particular relation are available (\ie, annotated), the benefit of pretraining on other relations evaporates. This result is surprising given the diversity of head entities available among the pretraining tuples. We would expect the model to see greater benefit from seeing many commonsense relationships during pretraining. Consequently, we conclude that annotating even a few examples of a new relation is the most fruitful way to improve a knowledge model's understanding of that relation.

However, it appears that knowledge models do manage to transfer some information between relations, with zero-shot relation induction improving drastically when the knowlege model is trained on other relations in the graph. However, this pretraining is only beneficial at scale. Restricted pretraining on only $n$ examples of the non-target relations performs the same as not pretraining (\legendtriangle).

% Interesting, we do find that pretraining on other relations is eff  zero-shot scores outperform the few-shot ($n=3$) setting for knowledge modeling, highlighting the utility of using an additional knowledge model for pretraining. 
